DDOTI Observations of Gravitational-Wave Sources Discovered in O3

We present optical follow-up observations with the DDOTI telescope of gravitational-wave events detected during the Advanced LIGO and Advanced Virgo O3 observing run. DDOTI is capable of responding to an alert in a few minutes, has an instantaneous field of about 69 deg$^{2}$, and obtains $10\sigma$ upper limits of $w_{\rm lim}=18.5$ to 20.5 AB mag in 1000~s of exposure, depending on the conditions. We observed 54\% (26 out of 48) of the unretracted gravitational-wave alerts and did not find any electromagnetic counterparts. We compare our upper limits to various possible counterparts: the kilonova AT~2017gfo, models of radioactive- and magnetar-powered kilonovae, short gamma-ray burst afterglows, and AGN flares. Although the large positional uncertainties of GW sources do not allow us to place strong constraints during O3, DDOTI observations of well-localized GW events in O4 and beyond could meaningfully constrain models of compact binary mergers. We show that DDOTI is able to detect kilonovae similar to AT~2017gfo up to about 200~Mpc and magnetar-powered kilonovae up to 1~Gpc. We calculate that nearby ($\lesssim$200 Mpc) afterglows have a high chance ($\approx$70\%) to be detected by rapid ($\lesssim$3 hours) DDOTI observations if observed on-axis, whereas off-axis afterglows are unlikely to be seen. Finally, we suggest that long-term monitoring of massive BBH events with DDOTI could confirm or rule out late AGN flares associated with these events.

==> DDOTI O3/TABLES/tablalims.tex <==
GW190408$\_$181802&17.30&18.60&0.04&186.39 -- 285.13\\
GW190412&26.85&21.25&0.14&42.28 -- 69.42\\
GW190421$\_$213856&34.10&18.95&0.01&205.61 -- 293.01\\
GW190425&2.25&19.75&0.01&19.86 -- 49.88\\
GW190426$\_$152155&19.85&20.70&0.14&64.71 -- 74.56\\
GW190513$\_$205418&12.70&19.40&0.03&92.05 -- 106.06\\
GW190521&4.25&20.10&0.01&21.67 -- 24.97\\
GW190521$\_$074359&1.95&20.03&0.01&14.86 -- 24.39\\
GW190706$\_$222641&7.65&20.75&$<0.01$&17.71 -- 25.24\\
GW190814&12.75&18.50&0.47&216.29 -- 287.16\\
GW190828$\_$063405&3.45&20.10&$<0.01$&22.55 -- 25.98\\
%S190910&6.00&18.50&0.02&96.28 -- 195.54\\
GW190915$\_$235702&51.10&19.45&0.03&221.80 -- 316.09\\
%S190923y&21.50&19.75&0.07&110.76 -- 181.88\\
GW190930$\_$133541&17.45&20.02&0.05&59.15 -- 97.13\\
S191105e&207.35&18.50&0.01&2076.17 -- 1022.28\\
S191109d&7.80&19.90&0.02&47.59 -- 54.83\\
S191204r&15.15&18.70&0.10&168.98 -- 297.84\\
S191205ah&5.00&18.50&0.09&102.38 -- 156.62\\
S191215w&4.15&19.60&$<0.01$&23.28 -- 72.32\\
S191216ap&5.85&19.55&0.27&56.30 -- 80.24\\
%%%%S200114f&5.10&19.85&0.64&
S200115j&1.45&18.20&0.05&58.23 -- 77.31\\
S200213t&1.60&19.25&0.15&23.78 -- 51.85\\
S200219ac&20.25&21.30&0.01&26.35 -- 34.98\\
S200224ca&8.45&21.00&0.23&20.66 -- 31.61\\
S200225q&0.25&18.45&0.01&12.42 -- 17.69\\
S200316bj&5.30&19.00&0.04&65.34 -- 99.95\\

==> DDOTI O3/TABLES/table-events2.tex <==
GW190408$\_$181802& BBH  &$\checkmark$&\\
GW190412& BBH  &$\checkmark$&\\
GW190421$\_$213856& BBH   &$\checkmark$& Bad weather\\
GW190425& BNS  &$\checkmark$&\\
GW190426$\_$152155& NSBH  &$\checkmark$&\\
GW190503$\_$185404& BBH  &            &Too far south\\
%S190510g & T (58\%) & & Low significance \\%?? & Low significance \\
GW190512$\_$180714& BBH  &            &Closed for maintenance\\
GW190513$\_$205428& BBH   &$\checkmark$&\\
GW190517$\_$055101& BBH   &            & Computer failed 20~m before event\\
GW190519$\_$153544& BBH  & &Bad weather (clouds)\\
GW190521& BBH   &$\checkmark$&\\
GW190521$\_$074359& BBH &$\checkmark$&\\
GW190602$\_$175927& BBH    &            &Too close to Sun\\
GW190630$\_$185205& BBH  &            &Closed for maintenance\\
GW190701$\_$203306& BBH   &            &Too close to Sun\\
GW190706$\_$222641& BBH   &$\checkmark$&\\
GW190707$\_$093326& BBH  &            &Bad weather (wind)\\
%S190718y&T (98\%)& $\checkmark$&   Bad weather (clouds) and low significance.\\
GW190720$\_$000836& BBH   &           & Poor initial localization\\
GW190727$\_$060333& BBH   &            &Bad weather (humidity)\\
GW190728$\_$064510& BBH   &            &Bad weather (humidity).\\
GW190814& MG &$\checkmark$&\\
GW190828$\_$063405& BBH  &$\checkmark$&\\
GW190828$\_$065509& BBH  &            & Priority given to GW190828$\_$063405\\
% Withdrawn: S190901ap&BNS (86\%)&          & Poor localization and low significance.\\
% Withdrawn: S190910d&NSBH (98\%)&$\checkmark$& Low significance.\\
% Withdrawn: S190910h&BNS (61\%)&            & Priority given to GW190910d and low significance.\\
GW190915$\_$235702& BBH   &$\checkmark$&\\
% Withdrawn: S190923y&NSBH (68\%)&$\checkmark$& Low significance. \\
GW190924$\_$021846& BBH   & & Close to Moon\\
GW190930$\_133541$& BBH    &$\checkmark$&\\
% Withdrawn: S190930t&NSBH (74\%)&   & Priority given to 190930s and low significance.\\
S191105e&BBH (95\%)&$\checkmark$&Alert delayed by about 28 h\\
S191109d&BBH (>99\%)&$\checkmark$&\\
S191129u&BBH (>99\%)&            &Poor initial localization\\
S191204r&BBH (>99\%)&$\checkmark$&\\
S191205ah&NSBH (93\%)&$\checkmark$&\\
S191213g&BNS (77\%)&            &Too close to Sun\\
S191215w&BBH (>99\%)&$\checkmark$&\\
S191216ap&BBH (99\%)&$\checkmark$&\\
S191222n&BBH (>99\%)&            &Bad weather (wind)\\
%S200105&T (>99\%)&            &OAN-closed\\
S200112r&BBH (>99\%)&            &Poor localization\\
S200114f& Burst        &$\checkmark$&\\
S200115j&MG (>99\%)&$\checkmark$&Bad weather (clouds)\\
S200128d&BBH (97\%)&            &Poor localization\\
S200129m&BBH (>99\%)&            &Too close to Sun\\
S200208q&BBH (99\%)&            &Too distant\\
S200213t&BNS (63\%)&$\checkmark$&\\
S200219ac&BBH (96\%)&$\checkmark$&\\
S200224ca&BBH (>99\%)&$\checkmark$&\\
S200225q&BBH (96\%)&$\checkmark$&\\
S200302c&BBH (89\%)&            &Poor localization\\
S200311bg&BBH (>99\%)&            &Too close to Sun\\
S200316bj&MG (>99\%)&$\checkmark$&\\

==> DDOTI O3/TABLES/table-observations.tex <==
GW190408$\_$181802&121&64&0.6&1&16.8--17.8&0.7&18.3--18.9&1550&BBH&\cite{2019GCN.24086....1W}\\
GW190412&69&33&1&2&24.1--29.6&4&20.9--21.6&740&BBH\\
GW190421$\_$213856&400&32&18.8&2&30.8--37.4&3.6&18.7--19.2&2880&BBH\\
&&&&3&54.0--61.2&4.1&19.0--19.4&&\\
GW190425&80&2&0.7&1&1.6--2.9&0.6&19.1--20.4&160&BNS\\
&&&&2&23.2--27.5&2.2&20.6--21.2&&\\
GW190426$\_$152155&384&25&0.2&1&12.2--27.5&7.8&20.6--20.8&370&NSBH&\cite{2019GCN.24310....1W}\\
GW190513$\_$205428&80&30&0.5&1&12.3--13.1&0.4&19.3--19.5&2060&BBH\\
GW190521&280&23&0.1&1&1.5--7.0&3.4&20.0--20.2&3920&BBH&\cite{2019GCN.24644....1W}\\
GW190521$\_$074359&80&9&0.1&1&0.2--3.7&0.8&19.7--20.4&1240&BBH\\
GW190706$\_$222641&67&5&0.3&1&5.8--9.5&2.4&20.5--21.0&4420&BBH\\
GW190814&100&95&0.5&1&10.8--14.7&1.1&18.3--18.7&240&MG&\cite{2019GCN.25352....1D}\\
&&&&2&34.8--38.8&1.3&18.4--18.9&&\\
&&&&4&82.7--86.7&1.9&18.4--18.9&&\\
&&&&5&108.6--110.7&1.5&18.7--19.2&&\\
&&&&6&134.4--134.8&0.3&18.9--19.1&&\\
&&&&7&154.4--158.8&3&19.6--19.8&&\\
&&&&13&301.5--302.8&0.9&20.6--20.8&&\\
&&&&14&322.0--322.3&0.3&19.5--20.0&&\\
&&&&21&489.7--493.9&2.1&19.9--20.6&&\\
&&&&25&585.7--591.1&3.3&20.6--21.0&&\\
&&&&26&609.6--613.3&2.2&20.1--20.7&&\\
GW190828$\_$063405&231&5&0.3&1&1.4--5.5&2.5&20.0--20.2&2130&BBH&\cite{2019GCN.25562....1P}\\
&&&&2&20.7--22.4&1.2&20.0--20.1&&\\
&&&&4&68.8--77.4&4.4&19.1-20.2&&\\
&&&&5&92.8--99.7&3.6&19.8--20.0&&\\
% Withdrawn: S190910d&28&11&0.1&1&3.0--9.0&3.4&18.0-19.0&606&BBH&\cite{2019GCN.25737....1P}\\
% Withdrawn: &&&&2&27.0--33.2&4.2&19.0--19.5&&\\
GW190915$\_$235702&80&27&0.1&3&50.9--51.3&0.3&19.2--19.7&1620&BBH\\

% Withdrawn: S190923y	& 183 &  12	&  0.1 &1  &  20.3--22.7 &1.6&	19.4--20.1 	&438&NSBH			\\


GW190930$\_$133541&80&6&0.1&1&13.0--21.9&5.7&20.0--20.7&760&BBH\\
S191105e&80&6&28.4&9&207.2--207.5&0.3&18.0--19.0&1183&BBH\\
S191109d&310&15&0.2&1&6.5-9.1&3.2&19.8--20.0&1810&BBH\\
&&&&2&24.8-32.8&4&18.8--19.5&&\\
&&&&3&47.9-56.1&4&19.9--20.4&&\\
&&&&4&72.9-73.6&0.7&17.2--17.9&&\\
S191204r&465&94&0.7&1&15.0-15.3&0.3&18.3--19.1&678&BBH\\
S191205ah&132&31&0.1&1&3.8-6.2&2.4&18.2--18.8&385&NSBH\\
S191215w&59&4&0.1&1&3.2-5.1&1.9&18.8--20.4&1779&BBH\\
&&&&6&125.1-125.5&0.2&17.4--18.7&&\\
S191216ap&313&63&0.3&1&4.8-6.9&1.9&19.3--19.8&376&BBH\\
&&&&2&28.3--31.3&1.8&19.8–20.3&&\\
&&&&4&76.3--76.8&1.9&18.5–19.4&&\\
&&&&5&101.0--101.3&0.8&17.7–18.9&&\\
S200114f&280&80&0.1&1&0.5-9.7&1.1&19.6--20.1&999&Burst&\cite{2020GCN.26752....1D}\\
&&&&2&24.3-24.6&0.3&18.1--18.9&&\\
&&&&5&97.9-103.9&6&20.0--20.8&&\\
S200115j&116&25&0.1&1&1.3-1.6&0.3&17.2--18.4&340&MG\\
&&&&2&22.0-23.3&0.8&20.0--20.1&&\\
S200213t&200&37&0.1&1&0.6-2.6&1.6&18.7-19.8&201&BNS&\cite{2020GCN.27061....1W}\\
&&&&2&22.3-25.1&1.9&18.3--19.8&&\\
&&&&3&46.3-46.9&0.6&18.7--19.2&&\\
S200219ac&320&16&2.6&1&17.8-22.7&6.2&21.1--21.5&3533&BBH\\
S200224ca&135&92&0.1&1&7.1-9.8&4.7&20.7--21.3&1575&BBH&\cite{2020GCN.27212....1D}\\
S200225q&432&27&0.1&1&0.1-0.4&0.2&18.2--18.7&995&BBH\\
S200316bj&81&40&0.1&1&4.8-5.8&1.7&18.7--19.3&1778&MG&\cite{2020GCN.27402....1P}\\

==> DDOTI O3/figurespng.tex <==

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure0.png}
 \caption{DDOTI observations of GW190408$\_$181802. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure1.png}
 \caption{DDOTI observations of GW190412. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations1}
\end{figure*}


\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure2.png}
 \contcaption{DDOTI observations of GW190421$\_$213856. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations2}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure3.png}
 \contcaption{DDOTI observations of GW190425. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations3}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure4.png}
 \contcaption{DDOTI observations of GW190426$\_$152155. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations4}
\end{figure*}


\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure5.png}
 \contcaption{DDOTI observations of GW190513$\_$205428. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations5}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure6.png}
 \contcaption{DDOTI observations of GW190521. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations6}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure7.png}
 \contcaption{DDOTI observations of GW190521$\_$074359. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
 \label{fig:observations7}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure8.png}
 \contcaption{DDOTI observations of GW190706$\_$222641. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}


 \label{fig:observations9}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure9.png}
 \contcaption{DDOTI observations of GW190814. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations10}
\end{figure*}




\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure10.png}
 \contcaption{DDOTI observations of GW190828$\_$063405. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations11}
\end{figure*}

%\begin{figure*}
%\centering
% \includegraphics[width=0.80\textwidth]{Figure11.png}
% \contcaption{DDOTI observations of S190910d. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

% \label{fig:observations12}
%\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure12.png}
 \contcaption{DDOTI observations of GW190915$\_$235702. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations13}
\end{figure*}

%\begin{figure*}
%\centering
% \includegraphics[width=0.80\textwidth]{Figure13.png}
% \contcaption{DDOTI observations of S190923y. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}
%
% \label{fig:observations14}
%\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure14.png}
 \contcaption{DDOTI observations of GW190930$\_$133541. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations15}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure15.png}
 \contcaption{DDOTI observations of S191105e. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations16}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure16.png}
 \contcaption{DDOTI observations of S191109d. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations17}
\end{figure*}


\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure17.png}
 \contcaption{DDOTI observations of S191204r. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations18}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure18.png}
 \contcaption{DDOTI observations of S191205ah. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations19}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure19.png}
 \contcaption{DDOTI observations of S191215w. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations20}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure20.png}
 \contcaption{DDOTI observations of S191216ap. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations21}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure21.png}
 \contcaption{DDOTI observations of S200114f. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations22}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure22.png}
 \contcaption{DDOTI observations of S200115j. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations23}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure23.png}
 \contcaption{DDOTI observations of S200213t. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations24}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure24.png}
 \contcaption{DDOTI observations of S200219ac. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations25}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure25.png}
 \contcaption{DDOTI observations of S200224ca. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations26}
\end{figure*}

\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure26.png}
 \contcaption{DDOTI observations of S200225q. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations27}
\end{figure*}


\begin{figure*}
\centering
 \includegraphics[width=0.80\textwidth]{FIGURES/Figure27.png}
 \contcaption{DDOTI observations of S200316bj. DDOTI fields are shown as orange quadrilaterals and the LIGO/Virgo probability map by blue and purple shading. The Sun and Moon (at the moment when DDOTI began to observe) are indicated by yellow and grey circles respectively. The black dashed line indicates the region of the sky available to DDOTI at the start of the night, the black dotted line indicates the region available to DDOTI at the end of the night, and the black solid line indicates the region available at some point during the night.}

 \label{fig:observations28}
\end{figure*}



==> DDOTI O3/references.tex <==
\bibitem[\protect\citeauthoryear{Abbott et al.}{2016a}]{Abbott2016a} Abbott B.~P., Abbott R., Abbott T.~D., Abernathy M.~R., Acernese F., Ackley K., Adams C., et al., 2016a, ApJL, 818, L22. doi:10.3847/2041-8205/818/2/L22

\bibitem[\protect\citeauthoryear{Abbott et al.}{2016b}]{Abbott2016b} Abbott B.~P., et al., 2016b, PhRvL, 116, 061102

\bibitem[\protect\citeauthoryear{Abbott et al.}{2017a}]{Abbott2017a} Abbott B.~P., et al., 2017a, PhRvL, 119, 161101

\bibitem[\protect\citeauthoryear{Abbott et al.}{2017b}]{Abbott2017b} Abbott B.~P., et al., 2017b, ApJL, 848, L12

\bibitem[\protect\citeauthoryear{Abbott, et al.}{2019}]{Abbott2019} Abbott B.~P., et al., 2019, PhRvD, 100, 064064

\bibitem[Abbott et al.(2020a)]{Abbott2020a} Abbott, B.~P., Abbott, R., Abbott, T.~D., et al.\ 2020a Living Reviews in Relativity, 23, 3. doi:10.1007/s41114-020-00026-9

\bibitem[\protect\citeauthoryear{Abbott et al.}{2020b}]{LVC190814} Abbott R., Abbott T.~D., Abraham S., Acernese F., Ackley K., Adams C., Adhikari R.~X., et al., 2020b, ApJL, 896, L44. doi:10.3847/2041-8213/ab960f

\bibitem[\protect\citeauthoryear{Abbott et al.}{2020c}]{Abbott2020c} Abbott R., Abbott T.~D., Abraham S., Acernese F., Ackley K., Adams A., Adams C., et al., 2020c, arXiv, arXiv:2010.14527

\bibitem[\protect\citeauthoryear{Abbott et al.}{2020d}]{LIGOpop} Abbott R., Abbott T.~D., Abraham S., Acernese F., Ackley K., et al., 2020d, arXiv, arXiv:2010.14533


\bibitem[\protect\citeauthoryear{Ackley et al.}{2020}]{Ackley2020} Ackley K., Amati L., Barbieri C., Bauer F.~E., Benetti S., Bernardini M.~G., Bhirombhakdi K., et al., 2020, A\&A, 643, A113. doi:10.1051/0004-6361/202037669

\bibitem[\protect\citeauthoryear{Ahn et al.}{2012}]{Ahn2012} Ahn C.~P., Alexandroff R., Allende Prieto C., Anderson S.~F., Anderton T., Andrews B.~H., Aubourg {\'E}., et al., 2012, ApJS, 203, 21. doi:10.1088/0067-0049/203/2/21

\bibitem[\protect\citeauthoryear{Alexander et al.}{2021}]{Alexander2021} Alexander K.~D., Schroeder G., Paterson K., Fong W., Cowperthwaite P., Gomez S., Margalit B., et al., 2021, arXiv, arXiv:2102.08957

\bibitem[\protect\citeauthoryear{Andreoni et al.}{2017}]{Andreoni2017} Andreoni I., Ackley K., Cooke J., Acharyya A., Allison J.~R., Anderson G.~E., Ashley M.~C.~B., et al., 2017, PASA, 34, e069. doi:10.1017/pasa.2017.65


\bibitem[Andreoni et al.(2020)]{Andreoni2020} Andreoni, I., Goldstein, D.~A., Kasliwal, M.~M., et al.\ 2020, \apj, 890, 131

\bibitem[\protect\citeauthoryear{Andreoni et al.}{2021}]{Andreoni2021} Andreoni I., Coughlin M.~W., Kool E.~C., Kasliwal M.~M., Kumar H., Bhalerao V., Sagu{\'e}s Carracedo A., et al., 2021, arXiv, arXiv:2104.06352

\bibitem[\protect\citeauthoryear{Antier et al.}{2020}]{Antier2020} Antier S., Agayeva S., Almualla M., Awiphan S., Baransky A., Barynova K., Beradze S., et al., 2020, MNRAS, 497, 5518. doi:10.1093/mnras/staa1846

\bibitem[\protect\citeauthoryear{Arcavi et al.}{2017}]{Arcavi2017} Arcavi I., Hosseinzadeh G., Howell D.~A., McCully C., Poznanski D., Kasen D., Barnes J., et al., 2017, Natur, 551, 64. doi:10.1038/nature24291

\bibitem[\protect\citeauthoryear{Ascenzi et al.}{2021}]{Ascenzi2021} Ascenzi S., Oganesyan G., Branchesi M., Ciolfi R., 2021, JPlPh, 87, 845870102. doi:10.1017/S0022377820001646

\bibitem[\protect\citeauthoryear{Barbieri et al.}{2019}]{Barbieri2019} Barbieri C., Salafia O.~S., Colpi M., Ghirlanda G., Perego A., Colombo A., 2019, ApJL, 887, L35. doi:10.3847/2041-8213/ab5c1e

\bibitem[\protect\citeauthoryear{Barbieri et al.}{2020}]{Barbieri2020} Barbieri C., Salafia O.~S., Colpi M., Ghirlanda G., Perego A., 2020, arXiv, arXiv:2002.09395

\bibitem[\protect\citeauthoryear{Bartos et al.}{2017}]{Bartos2017} Bartos I., Kocsis B., Haiman Z., M{\'a}rka S., 2017, ApJ, 835, 165. doi:10.3847/1538-4357/835/2/165

\bibitem[\protect\citeauthoryear{Becerra et al.}{2019}]{Becerra2019} Becerra R.~L., Dichiara S., Watson A.~M., Troja E., Fraija N., Klotz A., Butler N.~R., et al., 2019, ApJ, 881, 12. doi:10.3847/1538-4357/ab275b

\bibitem[\protect\citeauthoryear{Becerra et al.}{2021}]{Becerra2021} Becerra R.~L., De Colle F., Cant{\'o} J., Lizano S., Gonz{\'a}lez R.~F., Granot J., Klotz A., et al., 2021, ApJ, 908, 39. doi:10.3847/1538-4357/abcd3a

\bibitem[\protect\citeauthoryear{Beniamini \& van der Horst}{2017}]{BeniaminivanderHorst} Beniamini P., van der Horst A.~J., 2017, MNRAS, 472, 3161. doi:10.1093/mnras/stx2203

\bibitem[\protect\citeauthoryear{Bennett et al.}{2014}]{Bennett2014} Bennett C.~L., Larson D., Weiland J.~L., Hinshaw G., 2014, ApJ, 794, 135. doi:10.1088/0004-637X/794/2/135

\bibitem[\protect\citeauthoryear{Bernuzzi et al.}{2020}]{Bernuzzi2020} Bernuzzi S., Breschi M., Daszuta B., Endrizzi A., Logoteta D., Nedora V., Perego A., et al., 2020, MNRAS, 497, 1488. doi:10.1093/mnras/staa1860


\bibitem[\protect\citeauthoryear{Bertin \& Arnouts}{1996}]{Bertin1996} Bertin E., Arnouts S., 1996, A\&AS, 117, 393

\bibitem[\protect\citeauthoryear{Bertin}{2010}]{Bertin2010} Bertin E., 2010, Astrophysics Source Code Library, ascl:1010.068

\bibitem[\protect\citeauthoryear{Bruni et al.}{2021}]{Bruni2021} Bruni G., O'Connor B., Matsumoto T., Troja E., Piran T., Piro L., Ricci R., 2021, MNRAS.tmp. doi:10.1093/mnrasl/slab046

\bibitem[\protect\citeauthoryear{Chang et al.}{2021}]{Skymapper} Chang S.-W., Onken C.~A., Wolf C., Luvaul L., M{\"o}ller A., Scalzo R., Schmidt B.~P., et al., 2021, arXiv, arXiv:2102.07353

\bibitem[\protect\citeauthoryear{Chase et al.}{2021}]{Chase2021} Chase E.~A., O'Connor B., Fryer C.~L., Troja E., Korobkin O., Wollaeger R.~T., Ristic M., et al., 2021, arXiv, arXiv:2105.12268

\bibitem[\protect\citeauthoryear{Connaughton et al.}{2016}]{Connaughton2016} Connaughton V., Burns E., Goldstein A., Blackburn L., Briggs M.~S., Zhang B.-B., Camp J., et al., 2016, ApJL, 826, L6. doi:10.3847/2041-8205/826/1/L6

\bibitem[\protect\citeauthoryear{Coulter et al.}{2017}]{Coulter2017} Coulter D.~A., et al., 2017, Science, 358, 1556

\bibitem[\protect\citeauthoryear{Cromartie et al.}{2020}]{Cromartie2020} Cromartie H.~T., Fonseca E., Ransom S.~M., Demorest P.~B., Arzoumanian Z., Blumer H., Brook P.~R., et al., 2020, NatAs, 4, 72. doi:10.1038/s41550-019-0880-2

\bibitem[\protect\citeauthoryear{Darbha \& Kasen}{2020}]{Darbha2020} Darbha S., Kasen D., 2020, ApJ, 897, 150. doi:10.3847/1538-4357/ab9a34

\bibitem[\protect\citeauthoryear{D{\'\i}az et al.}{2017}]{Diaz2017} D{\'\i}az M.~C., Macri L.~M., Garcia Lambas D., Mendes de Oliveira C., Nilo Castell{\'o}n J.~L., Ribeiro T., S{\'a}nchez B., et al., 2017, ApJL, 848, L29. doi:10.3847/2041-8213/aa9060

\bibitem[\protect\citeauthoryear{Dichiara et al.}{2019}]{2019GCN.25352....1D} Dichiara S., Pereyra M., Watson A.~M., Butler N., Becerra R.~L., Gonzalez D., Kutyrev A., et al., 2019, GCN, 25352

\bibitem[\protect\citeauthoryear{Dichiara \& Wolfram}{2020}]{2020GCN.26752....1D} Dichiara S., Wolfram T., 2020, GCN, 26752, 1

\bibitem[\protect\citeauthoryear{Dichiara, et al.}{2020a}]{2020GCN.27212....1D} Dichiara S., et al., 2020a, GCN, 27212, 1

\bibitem[\protect\citeauthoryear{Dichiara et al.}{2020b}]{Dichiara2020} Dichiara S., Troja E., O'Connor B., Marshall F.~E., Beniamini P., Cannizzo J.~K., Lien A.~Y., et al., 2020b, MNRAS, 492, 5011. doi:10.1093/mnras/staa124

\bibitem[\protect\citeauthoryear{Dichiara et al.}{2021}]{Dichiara2021} Dichiara S., Troja E., Beniamini P., O'Connor B., Moss M., Lien A.~Y., Ricci R., et al., 2021, ApJL, 911, L28. doi:10.3847/2041-8213/abf562

\bibitem[\protect\citeauthoryear{Dobie et al.}{2019}]{Dobie2019} Dobie D., Stewart A., Murphy T., Lenc E., Wang Z., Kaplan D.~L., Andreoni I., et al., 2019, ApJL, 887, L13. doi:10.3847/2041-8213/ab59db

\bibitem[\protect\citeauthoryear{Estell{\'e}s et al.}{2021}]{Estelle2021} Estell{\'e}s H., Husa S., Colleoni M., Mateu-Lucena M., de Lluc Planas M., Garc{\'\i}a-Quir{\'o}s C., Keitel D., et al., 2021, arXiv, arXiv:2105.06360


\bibitem[\protect\citeauthoryear{Evans et al.}{2016}]{Evans2016} Evans P.~A., Kennea J.~A., Palmer D.~M., Bilicki M., Osborne J.~P., O'Brien P.~T., Tanvir N.~R., et al., 2016, MNRAS, 462, 1591. doi:10.1093/mnras/stw1746


\bibitem[\protect\citeauthoryear{Evans et al.}{2017}]{Evans2017} Evans P.~A., Cenko S.~B., Kennea J.~A., Emery S.~W.~K., Kuin N.~P.~M., Korobkin O., Wollaeger R.~T., et al., 2017, Sci, 358, 1565. doi:10.1126/science.aap9580

\bibitem[\protect\citeauthoryear{Fern{\'a}ndez, Foucart, \& Lippuner}{2020}]{Fernandez2020} Fern{\'a}ndez R., Foucart F., Lippuner J., 2020, MNRAS, 497, 3221. doi:10.1093/mnras/staa2209

\bibitem[\protect\citeauthoryear{Fontes et al.}{2020}]{Fontes2020} Fontes C.~J., Fryer C.~L., Hungerford A.~L., Wollaeger R.~T., Korobkin O., 2020, MNRAS, 493, 4143. doi:10.1093/mnras/staa485

\bibitem[\protect\citeauthoryear{Fujibayashi et al.}{2020}]{Fujibashi2020} Fujibayashi S., Wanajo S., Kiuchi K., Kyutoku K., Sekiguchi Y., Shibata M., 2020, ApJ, 901, 122. doi:10.3847/1538-4357/abafc2

\bibitem[\protect\citeauthoryear{Gao \& Fan}{2006}]{Gao2006} Gao W.-H., Fan Y.-Z., 2006, ChJAA, 6, 513. doi:10.1088/1009-9271/6/5/01

\bibitem[\protect\citeauthoryear{Gao et al.}{2017}]{Gao2017} Gao H., Zhang B., L{\"u} H.-J., Li Y., 2017, ApJ, 837, 50. doi:10.3847/1538-4357/aa5be3

\bibitem[\protect\citeauthoryear{Gehrels et al.}{2016}]{Gehrels2016} Gehrels N., Cannizzo J.~K., Kanner J., Kasliwal M.~M., Nissanke S., Singer L.~P., 2016, ApJ, 820, 136. doi:10.3847/0004-637X/820/2/136

\bibitem[\protect\citeauthoryear{Goldstein, et al.}{2017}]{Goldstein2017} Goldstein A., et al., 2017, ApJL, 848, L14

\bibitem[\protect\citeauthoryear{Golkhou et al.}{2018}]{Golkhou2018} Golkhou V.~Z., Butler N.~R., Strausbaugh R., Troja E., Kutyrev A., Lee W.~H., Rom{\'a}n-Z{\'u}{\~n}iga C.~G., et al., 2018, ApJ, 857, 81. doi:10.3847/1538-4357/aab665


\bibitem[\protect\citeauthoryear{Gompertz et al.}{2020}]{Gompertz2020} Gompertz B.~P., Cutter R., Steeghs D., Galloway D.~K., Lyman J., Ulaczyk K., Dyer M.~J., et al., 2020, MNRAS, 497, 726. doi:10.1093/mnras/staa1845

\bibitem[\protect\citeauthoryear{Graham et al.}{2020}]{Graham2020} Graham M.~J., Ford K.~E.~S., McKernan B., Ross N.~P., Stern D., Burdge K., Coughlin M., et al., 2020, PhRvL, 124, 251102. doi:10.1103/PhysRevLett.124.251102

\bibitem[\protect\citeauthoryear{Granot, De Colle, \& Ramirez-Ruiz}{2018}]{Granot2018} Granot J., De Colle F., Ramirez-Ruiz E., 2018, MNRAS, 481, 2711. doi:10.1093/mnras/sty2454

%\bibitem[\protect\citeauthoryear{Haggard et al.}{2017}]{Haggard2017} Haggard D., Nynka M., Ruan J.~J., Kalogera V., Cenko S.~B., Evans P., Kennea J.~A., 2017, ApJL, 848, L25. doi:10.3847/2041-8213/aa8ede

\bibitem[\protect\citeauthoryear{Hallinan et al.}{2017}]{Hallinan2017} Hallinan G., Corsi A., Mooley K.~P., Hotokezaka K., Nakar E., Kasliwal M.~M., Kaplan D.~L., et al., 2017, Sci, 358, 1579. doi:10.1126/science.aap9855


\bibitem[\protect\citeauthoryear{Henden et al.}{2018}]{Henden2018} Henden A.~A., Levine S., Terrell D., Welch D.~L., Munari U., Kloppenborg B.~K., 2018, AAS, 232, 223.06

\bibitem[\protect\citeauthoryear{Hu et al.}{2017}]{Hu2017} Hu L., Wu X., Andreoni I., Ashley M.~C.~B., Cooke J., Cui X., Du F., et al., 2017, SciBu, 62, 1433. doi:10.1016/j.scib.2017.10.006

\bibitem[\protect\citeauthoryear{Jiang et al.}{2019}]{Jiang2019} Jiang Y.-F., Blaes O., Stone J.~M., Davis S.~W., 2019, ApJ, 885, 144. doi:10.3847/1538-4357/ab4a00

\bibitem[\protect\citeauthoryear{Kawaguchi et al.}{2015}]{Kawaguchi2015} Kawaguchi K., Kyutoku K., Nakano H., Okawa H., Shibata M., Taniguchi K., 2015, PhRvD, 92, 024014. doi:10.1103/PhysRevD.92.024014

\bibitem[\protect\citeauthoryear{Kawaguchi et al.}{2020}]{Kawaguchi2020} Kawaguchi K., Fujibayashi S., Shibata M., Tanaka M., Wanajo S., 2020, arXiv, arXiv:2012.14711


\bibitem[\protect\citeauthoryear{Klingler et al.}{2021}]{Klinger2021} Klingler N.~J., Lien A., Oates S.~R., Kennea J.~A., Evans P.~A., Tohuvavohu A., Zhang B., et al., 2021, ApJ, 907, 97. doi:10.3847/1538-4357/abd2c3

\bibitem[\protect\citeauthoryear{Korobkin et al.}{2021}]{Korobkin2021} Korobkin O., Wollaeger R.~T., Fryer C.~L., Hungerford A.~L., Rosswog S., Fontes C.~J., Mumpower M.~R., et al., 2021, ApJ, 910, 116. doi:10.3847/1538-4357/abe1b5

\bibitem[\protect\citeauthoryear{Kr{\"u}ger \& Foucart}{2020}]{Kruger2020} Kr{\"u}ger C.~J., Foucart F., 2020, PhRvD, 101, 103002. doi:10.1103/PhysRevD.101.103002

\bibitem[Kumar \& Zhang(2015)]{Kumar2015} Kumar, P. \& Zhang, B.\ 2015, \physrep, 561, 1. doi:10.1016/j.physrep.2014.09.008

\bibitem[\protect\citeauthoryear{Lang, et al.}{2010}]{Lang2010} Lang D., Hogg D.~W., Mierle K., Blanton M., Roweis S., 2010, AJ, 139, 1782

\bibitem[\protect\citeauthoryear{Lazzati et al.}{2018}]{Lazzati2018} Lazzati D., Perna R., Morsony B.~J., Lopez-Camara D., Cantiello M., Ciolfi R., Giacomazzo B., et al., 2018, PhRvL, 120, 241103. doi:10.1103/PhysRevLett.120.241103

\bibitem[\protect\citeauthoryear{Liu, Gao, \& Zhang}{2020}]{Li2020} Liu L.-D., Gao H., Zhang B., 2020, ApJ, 890, 102. doi:10.3847/1538-4357/ab6b24

\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration, et al.}{2015}]{LVC15} LIGO Scientific Collaboration, et al., 2015, CQGra, 32, 074001

\bibitem[\protect\citeauthoryear{Lipunov et al.}{2017}]{Lipunov2017} Lipunov V.~M., Gorbovskoy E., Kornilov V.~G., . Tyurina N., Balanutsa P., Kuznetsov A., Vlasenko D., et al., 2017, ApJL, 850, L1. doi:10.3847/2041-8213/aa92c0

\bibitem[\protect\citeauthoryear{L{\"u} et al.}{2015}]{Lu2015} L{\"u} H.-J., Zhang B., Lei W.-H., Li Y., Lasky P.~D., 2015, ApJ, 805, 89. doi:10.1088/0004-637X/805/2/89

\bibitem[\protect\citeauthoryear{McKernan et al.}{2020}]{McKernan2020} McKernan B., Ford K.~E.~S., O'Shaugnessy R., Wysocki D., 2020, MNRAS, 494, 1203. doi:10.1093/mnras/staa740

\bibitem[\protect\citeauthoryear{Miller et al.}{2019}]{Miller2019} Miller M.~C., Lamb F.~K., Dittmann A.~J., Bogdanov S., Arzoumanian Z., Gendreau K.~C., Guillot S., et al., 2019, ApJL, 887, L24. doi:10.3847/2041-8213/ab50c5

\bibitem[Monet et al.(2003)]{Monet2003} Monet, D.~G., Levine, S.~E., Canzian, B., et al.\ 2003, \aj, 125, 984. doi:10.1086/345888

\bibitem[\protect\citeauthoryear{Morgan et al.}{2020}]{Morgan2020} Morgan R., Soares-Santos M., Annis J., Herner K., Garcia A., Palmese A., Drlica-Wagner A., et al., 2020, ApJ, 901, 83. doi:10.3847/1538-4357/abafaa

\bibitem[\protect\citeauthoryear{Most et al.}{2020}]{Most2020} Most E.~R., Papenfort L.~J., Tootle S., Rezzolla L., 2020, arXiv, arXiv:2012.03896

\bibitem[\protect\citeauthoryear{Nakar}{2020}]{Nakar2020} Nakar E., 2020, PhR, 886, 1. doi:10.1016/j.physrep.2020.08.008

\bibitem[\protect\citeauthoryear{O'Connor, Beniamini, \& Kouveliotou}{2020}]{Oconnor2020} O'Connor B., Beniamini P., Kouveliotou C., 2020, MNRAS, 495, 4782. doi:10.1093/mnras/staa1433

\bibitem[\protect\citeauthoryear{O'Connor et al.}{2021}]{Oconnor2021} O'Connor B., Troja E., Dichiara S., Chase E.~A., Ryan G., Cenko S.~B., Fryer C.~L., et al., 2021, MNRAS, 502, 1279. doi:10.1093/mnras/stab132

\bibitem[\protect\citeauthoryear{Page et al.}{2020}]{Page2020} Page K.~L., Evans P.~A., Tohuvavohu A., Kennea J.~A., Klingler N.~J., Cenko S.~B., Oates S.~R., et al., 2020, MNRAS, 499, 3459. doi:10.1093/mnras/staa3032

%\bibitem[\protect\citeauthoryear{Pereyra, et al.}{2019a}]{2019GCN.25737....1P} Pereyra M., et al., 2019a, GCN, 25737, 1

\bibitem[\protect\citeauthoryear{Pereyra, et al.}{2019}]{2019GCN.25562....1P} Pereyra M., et al., 2019, GCN, 25562, 1

\bibitem[\protect\citeauthoryear{Pereyra, et al.}{2020}]{2020GCN.27402....1P} Pereyra M., et al., 2020, GCN, 27402, 1

\bibitem[\protect\citeauthoryear{Perna, Lazzati, \& Giacomazzo}{2016}]{Perna2016} Perna R., Lazzati D., Giacomazzo B., 2016, ApJL, 821, L18. doi:10.3847/2041-8205/821/1/L18

\bibitem[\protect\citeauthoryear{Pian et al.}{2017}]{Pian2017} Pian E., D'Avanzo P., Benetti S., Branchesi M., Brocato E., Campana S., Cappellaro E., et al., 2017, Natur, 551, 67. doi:10.1038/nature24298

\bibitem[\protect\citeauthoryear{Ricci et al.}{2021}]{Ricci2021} Ricci R., Troja E., Bruni G., Matsumoto T., Piro L., O'Connor B., Piran T., et al., 2021, MNRAS, 500, 1708. doi:10.1093/mnras/staa3241

\bibitem[\protect\citeauthoryear{Riley et al.}{2019}]{Riley2019} Riley T.~E., Watts A.~L., Bogdanov S., Ray P.~S., Ludlam R.~M., Guillot S., Arzoumanian Z., et al., 2019, ApJL, 887, L21. doi:10.3847/2041-8213/ab481c

\bibitem[\protect\citeauthoryear{Rowlinson et al.}{2013}]{Rowlinson2013} Rowlinson A., O'Brien P.~T., Metzger B.~D., Tanvir N.~R., Levan A.~J., 2013, MNRAS, 430, 1061. doi:10.1093/mnras/sts683

\bibitem[\protect\citeauthoryear{Ryan et al.}{2020}]{Ryan2020} Ryan G., van Eerten H., Piro L., Troja E., 2020, ApJ, 896, 166. doi:10.3847/1538-4357/ab93cf

\bibitem[\protect\citeauthoryear{Sagu{\'e}s Carracedo et al.}{2021}]{Sagues2021} Sagu{\'e}s Carracedo A., Bulla M., Feindt U., Goobar A., 2021, MNRAS, 504, 1294. doi:10.1093/mnras/stab872

\bibitem[\protect\citeauthoryear{Santana, Barniol Duran, \& Kumar}{2014}]{Santana14} Santana R., Barniol Duran R., Kumar P., 2014, ApJ, 785, 29. doi:10.1088/0004-637X/785/1/29

\bibitem[\protect\citeauthoryear{Sarin \& Lasky}{2020}]{Sarin2020} Sarin N., Lasky P.~D., 2020, arXiv, arXiv:2012.08172

\bibitem[\protect\citeauthoryear{Savchenko et al.}{2016}]{Savchenko2016} Savchenko V., Ferrigno C., Mereghetti S., Natalucci L., Bazzano A., Bozzo E., Brandt S., et al., 2016, ApJL, 820, L36. doi:10.3847/2041-8205/820/2/L36

\bibitem[\protect\citeauthoryear{Savchenko et al.}{2017}]{Savchenko2017} Savchenko V., Ferrigno C., Kuulkers E., Bazzano A., Bozzo E., Brandt S., Chenevez J., et al., 2017, ApJL, 848, L15. doi:10.3847/2041-8213/aa8f94

\bibitem[\protect\citeauthoryear{Schutz}{2011}]{Schutz2011} Schutz B.~F., 2011, CQGra, 28, 125023. doi:10.1088/0264-9381/28/12/125023

\bibitem[\protect\citeauthoryear{Singer \& Price}{2016}]{Singer2016} Singer L.~P., Price L.~R., 2016, PhRvD, 93, 024013. doi:10.1103/PhysRevD.93.024013

\bibitem[\protect\citeauthoryear{Soares-Santos et al.}{2017}]{Soares2017} Soares-Santos M., Holz D.~E., Annis J., Chornock R., Herner K., Berger E., Brout D., et al., 2017, ApJL, 848, L16. doi:10.3847/2041-8213/aa9059


\bibitem[\protect\citeauthoryear{Tanvir et al.}{2017}]{Tanvir2017} Tanvir N.~R., Levan A.~J., Gonz{\'a}lez-Fern{\'a}ndez C., Korobkin O., Mandel I., Rosswog S., Hjorth J., et al., 2017, ApJL, 848, L27. doi:10.3847/2041-8213/aa90b6

\bibitem[\protect\citeauthoryear{Thakur et al.}{2020}]{Thakur2020} Thakur A.~L., Dichiara S., Troja E., Chase E.~A., S{\'a}nchez-Ram{\'\i}rez R., Piro L., Fryer C.~L., et al., 2020, MNRAS, 499, 3868. doi:10.1093/mnras/staa2798

\bibitem[Tonry et al.(2012)]{Tonry2012} Tonry, J.~L., Stubbs, C.~W., Lykke, K.~R., et al.\ 2012, \apj, 750, 99. doi:10.1088/0004-637X/750/2/99

\bibitem[\protect\citeauthoryear{Troja et al.}{2016}]{Troja2016} Troja E., Read A.~M., Tiengo A., Salvaterra R., 2016, ApJL, 822, L8. doi:10.3847/2041-8205/822/1/L8

\bibitem[\protect\citeauthoryear{Troja et al.}{2017}]{Troja2017} Troja E., Piro L., van Eerten H., Wollaeger R.~T., Im M., Fox O.~D., Butler N.~R., et al., 2017, Natur, 551, 71. doi:10.1038/nature24290

\bibitem[\protect\citeauthoryear{Troja et al.}{2019}]{Troja19} Troja E., van Eerten H., Ryan G., Ricci R., Burgess J.~M., Wieringa M.~H., Piro L., et al., 2019, MNRAS, 489, 1919. doi:10.1093/mnras/stz2248


\bibitem[\protect\citeauthoryear{Typel et al.}{2010}]{Typel2010} Typel S., R{\"o}pke G., Kl{\"a}hn T., Blaschke D., Wolter H.~H., 2010, PhRvC, 81, 015803. doi:10.1103/PhysRevC.81.015803

\bibitem[\protect\citeauthoryear{Urrutia et al.}{2021}]{Urrutia2021} Urrutia G., De Colle F., Murguia-Berthier A., Ramirez-Ruiz E., 2021, MNRAS, 503, 4363. doi:10.1093/mnras/stab723

\bibitem[\protect\citeauthoryear{Utsumi et al.}{2017}]{Utsumi2017} Utsumi Y., Tanaka M., Tominaga N., Yoshida M., Barway S., Nagayama T., Zenko T., et al., 2017, PASJ, 69, 101. doi:10.1093/pasj/psx118

\bibitem[\protect\citeauthoryear{Valenti et al.}{2017}]{Valenti2017} Valenti S., Sand D.~J., Yang S., Cappellaro E., Tartaglia L., Corsi A., Jha S.~W., et al., 2017, ApJL, 848, L24. doi:10.3847/2041-8213/aa8edf

\bibitem[\protect\citeauthoryear{Veitch et al.}{2015}]{Veitch2015} Veitch J., Raymond V., Farr B., Farr W., Graff P., Vitale S., Aylott B., et al., 2015, PhRvD, 91, 042003. doi:10.1103/PhysRevD.91.042003

\bibitem[\protect\citeauthoryear{Vieira et al.}{2020}]{Vieira2020} Vieira N., Ruan J.~J., Haggard D., Drout M.~R., Nynka M.~C., Boyce H., Spekkens K., et al., 2020, ApJ, 895, 96. doi:10.3847/1538-4357/ab917d

\bibitem[\protect\citeauthoryear{Wang et al.}{2015}]{Wang2015} Wang X.-G., Zhang B., Liang E.-W., Gao H., Li L., Deng C.-M., Qin S.-M., et al., 2015, ApJS, 219, 9. doi:10.1088/0067-0049/219/1/9

\bibitem[\protect\citeauthoryear{Watson et al.}{2016}]{Watson2016} Watson A.~M., et al., 2016b, SPIE, 99100G

\bibitem[\protect\citeauthoryear{Watson et al.}{2019c}]{2019GCN.24086....1W} Watson A.~M., et al., 2019a, GCN, 24086, 1

\bibitem[\protect\citeauthoryear{Watson et al.}{2019b}]{2019GCN.24310....1W} Watson A.~M., et al., 2019b, GCN, 24310, 1

\bibitem[\protect\citeauthoryear{Watson, et al.}{2019a}]{2019GCN.24644....1W} Watson A.~M., et al., 2019c, GCN, 24644, 1

\bibitem[\protect\citeauthoryear{Watson et al.}{2020a}]{Watson2020} Watson A.~M., et al., 2020a, MNRAS, 492, 5916

\bibitem[\protect\citeauthoryear{Watson}{2020b}]{2020GCN.27061....1W} Watson A.~M., 2020b, GCN, 27061, 1

\bibitem[\protect\citeauthoryear{Wollaeger et al.}{2018}]{Wollaeger2018} Wollaeger R.~T., Korobkin O., Fontes C.~J., Rosswog S.~K., Even W.~P., Fryer C.~L., Sollerman J., et al., 2018, MNRAS, 478, 3298. doi:10.1093/mnras/sty1018

\bibitem[\protect\citeauthoryear{Wollaeger et al.}{2021}]{Wollaeger2021} Wollaeger R.~T., Fryer C.~L., Chase E.~A., Fontes C.~J., Ristic M., Hungerford A.~L., Korobkin O., et al., 2021, arXiv, arXiv:2105.11543

\bibitem[\protect\citeauthoryear{Yang et al.}{2019}]{Yang2019} Yang Y., Bartos I., Gayathri V., Ford K.~E.~S., Haiman Z., Klimenko S., Kocsis B., et al., 2019, PhRvL, 123, 181101. doi:10.1103/PhysRevLett.123.181101

\bibitem[\protect\citeauthoryear{Yi \& Cheng}{2019}]{Yi2019} Yi S.-X., Cheng K.~S., 2019, ApJL, 884, L12. doi:10.3847/2041-8213/ab459a


\bibitem[\protect\citeauthoryear{Yuan et al.}{2021}]{Yuan2021} Yuan Y., L{\"u} H.-J., Yuan H.-Y., Ma S.-B., Lei W.-H., Liang E.-W., 2021, arXiv, arXiv:2103.05811

\bibitem[\protect\citeauthoryear{Yu, Zhang, \& Gao}{2013}]{2013Yu} Yu Y.-W., Zhang B., Gao H., 2013, ApJL, 776, L40. doi:10.1088/2041-8205/776/2/L40

\bibitem[\protect\citeauthoryear{Zhang}{2016}]{Zhang2016} Zhang B., 2016, ApJL, 827, L31. doi:10.3847/2041-8205/827/2/L31

\bibitem[\protect\citeauthoryear{Zhang}{2019}]{Zhang2019} Zhang B., 2019, ApJL, 873, L9. doi:10.3847/2041-8213/ab0ae8

\bibitem[\protect\citeauthoryear{Zou et al.}{2018}]{Zou2018} Zou Y.-C., Wang F.-F., Moharana R., Liao B., Chen W., Wu Q., Lei W.-H., et al., 2018, ApJL, 852, L1. doi:10.3847/2041-8213/aaa123

%%%%%%%%%%%%%%%%%%%%%%%%        DDOTI GCNs            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%          




%%%%%%%%%%%%%%%%%%%%%%%%      LIGO  GCNs            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%          

\begin{comment}


\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24069....1L} Ligo Scientific Collaboration, \& VIRGO Collaboration\ 2019, GRB Coordinates Network 24069, 1
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24098....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24098
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24141....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24141
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24168....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN24168, \#1 (2019/April-0), 24168
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24237....1L} Ligo Scientific Collaboration, \& VIRGO Collaboration\ 2019, GRB Coordinates Network 24237, 1
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24377....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24377
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24442....1L} Ligo Scientific Collaboration, \& VIRGO Collaboration\ 2019, GRB Coordinates Network 24442, 1
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24503....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24503
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24522....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24522
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24570....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24570
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24598....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, \#1 (2019/May-0), 24598
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24621....1L} Ligo Scientific Collaboration, \& VIRGO Collaboration\ 2019, GRB Coordinates Network 24621, 1
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24632....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24632
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24717....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24717
\bibitem[\protect\citeauthoryear{Ligo Scientific Collaboration \& VIRGO Collaboration}{2019}]{2019GCN.24922....1L} Ligo Scientific Collaboration, VIRGO Collaboration, 2019, GCN, 24922
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24950....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 24950
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.24998....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN2, 24998
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25012....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25012
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25115....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25115
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25164....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25164
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25187....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25187
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25324....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2019, GRB Coordinates Network 25324, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25333....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2019, GRB Coordinates Network 25333, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25497....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25497
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25503....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25503
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25606....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25606
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25695....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2019, GRB Coordinates Network 25695, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25707....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25707
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25753....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25753. doi:10.1007/s11433-010-4137-4
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25814....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 25814
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25829....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 25829
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25871....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25871
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.25876....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2019, GCN, 25876
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26182....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26182
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26202....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26202
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26303....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26303
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26334....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN26334, 26334
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26350....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN26350, 26350
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26395....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2019, GRB Coordinates Network 26395, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26402....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26402
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26441....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN26441, 26441
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26454....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26454
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26513....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2019, GRB Coordinates Network 26513, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2019}]{2019GCN.26543....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2019, GCN, 26543
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26640....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN, 26640
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26715....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN, 26715
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26734....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2020, GRB Coordinates Network 26734, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26759....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2020, GRB Coordinates Network 26759, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26906....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN, 26906
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.26926....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN, 26926
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27014....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2020, GCN, 27014
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27042....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2020, GRB Coordinates Network 27042, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27130....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN27130, 27130
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27184....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2020, GRB Coordinates Network 27184, 1
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27193....1L} LIGO Scientific Collaboration, Virgo Collaboration\ 2020, GCN27193, 27193
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27278....1L} LIGO Scientific Collaboration, Virgo Collaboration, 2020, GCN, 27278
\bibitem[\protect\citeauthoryear{LIGO Scientific Collaboration \& Virgo Collaboration}{2020}]{2020GCN.27388....1L} LIGO Scientific Collaboration, \& Virgo Collaboration\ 2020, GRB Coordinates Network 27388, 1

\end{comment}

















